A Multi-Tenant Framework for Cloud Container Services

Container technologies have been evolving rapidly in the cloud-native era. Kubernetes, as a production-grade container orchestration platform, has been proven to be successful at managing containerized applications in on-premises datacenters. However, Kubernetes lacks sufficient multi-tenant supports by design, meaning in cloud environments, dedicated clusters are required to serve multiple users, i.e., tenants. This limitation significantly diminishes the benefits of cloud computing, and makes it difficult to build multi-tenant software as a service (SaaS) products using Kubernetes. In this paper, we propose Virtual-Cluster, a new multi-tenant framework that extends Kubernetes with adequate multi-tenant supports. Basically, VirtualCluster provides both control plane and data plane isolations while sharing the underlying compute resources among tenants. The new framework preserves the API compatibility by avoiding modifying the Kubernetes core components. Hence, it can be easily integrated with existing Kubernetes use cases. Our experimental results show that the overheads introduced by VirtualCluster, in terms of latency and throughput, is moderate.

==> availability.tex <==
\section*{Availability}
\label{sec:availability}

VC is an incubator project under the SIG-multitenancy working group of the 
Kubernetes community. The source code is hosted as a public Github 
Repository.


==> discussion.tex <==
\section{Discussion Topics}
Multi-tenancy in Kubernetes has increasingly gained people's interests 
since Kubernetes has become more and more popular.
A recent poll in KubeCon 2019 multi-tenancy working group panel shows that
at least half of the audiences (over hundreds of which) have multi-tenant requirements
in their environments. However, the fact is that users desire serverless
experiences with strong isolation 
but Kubernetes itself has quite some limitations in terms of hard multi-tenancy. 
We expect our work will stimulate at least the following discussions:
\\\\
\noindent {\bf 1. Should we pursue resolving the multi-tenant problems in upstream or
building our own solutions?} \\
This question often leads to debates since Kubernetes is 
an open-source project. We can share the feedbacks when discussing this with Kubernetes 
apimachinery tech leaders and their thoughts about VirtualCluster as well.
In short, the attempt to change core APIs is hard to realize. The core team
encourages all API enchancements through CRDs.
We can discuss the concerns of the audiences and see
whether they should be addressed in upstream or resolved in solutions like VirtualCluster.
\\\\
\noindent {\bf 2. What is the tenant master overhead in VirtualCluster? and how to
reduce it?}\\
It depends. For a few or dozens of
tenants, the tenant master cost should not be a big concern. However, such cost
can be a blocking issue if the
number of tenants reaches thousands or more. We have thought about how to 
reduce the tenant master cost and would like to discuss the applicability with the audiences.
\\\\
\noindent {\bf 3. Will the syncer controller be a source of contention?}\\
This question arises for any centralized hub in distributed systems. In VirtualCluster,
the syncer needs to distribute requests from all tenant masters. We do consider 
some contention problems when designing the syncer but not all of them. 
This discussion can help us refine our design.
\\\\
\noindent {\bf 4. What are the things that VirtualCluster does not support?}\\
Some Kubernetes workloads can work in 
VirtualCluster but we should not support, such as DaemonSet.
In a serverless model, node related API supports are restricted, such as
adding node labels or annotations. Currently, VirtualCluster does
not allow users to mutate the virtual node object.
This question can help clarify various VirtualCluster use cases.
\\\\
\noindent {\bf 5. Is the resource syncer extendable?} \\
Currently, no. But we do see the value of extending the syncer to support more resource
types or CRDs. We would like to get feedback about this and evaluate the urgency of such need. 


==> fair-queueing.tex <==
\begin{figure}[t]
\centering
\captionsetup{justification=centering}
\captionsetup[subfigure]{justification=centering}

\begin{subfigure}[b]{\linewidth}
\centering
\includegraphics[width=\linewidth]{unfair-tenants-with-fq.png}
\caption{With Fair Queue}
\label{fig:with-fair-queue}
\end{subfigure}

\begin{subfigure}[b]{\linewidth}
\centering
\includegraphics[width=\linewidth]{unfair-tenants-no-fq.png}
\caption{Without Fair Queue}
\label{fig:without-fair-queue}
\end{subfigure}

\caption{The Average Pod Creation Time \\ with and without the Fair Queueing}
\label{fig:fair-queueing}
\end{figure}


==> pod-creation-benchmark.tex <==
\begin{figure*}
{\centering
    \begin{tabular}{c@{}c@{}c@{}c}
{\centering {\bf 25 Tenants}} \smallskip & {\centering {\bf 50 Tenants}} \smallskip & {\centering {\bf 100 Tenants}} \smallskip \\
\includegraphics[width=0.33\textwidth]{25tenants1250pods.png} & \includegraphics[width=0.33\textwidth]{50tenants1250pods.png} & \includegraphics[width=0.33\textwidth]{100tenants1250pods.png} \\
\includegraphics[width=0.33\textwidth]{25tenants2500pods.png} & \includegraphics[width=0.33\textwidth]{50tenants2500pods.png} & \includegraphics[width=0.33\textwidth]{100tenants2500pods.png} \\
\includegraphics[width=0.33\textwidth]{25tenants5000pods.png} & \includegraphics[width=0.33\textwidth]{50tenants5000pods.png} & \includegraphics[width=0.33\textwidth]{100tenants5000pods.png} \\
\includegraphics[width=0.33\textwidth]{25tenants10000pods.png} & \includegraphics[width=0.33\textwidth]{50tenants10000pods.png} & \includegraphics[width=0.33\textwidth]{100tenants10000pods.png} \\
\end{tabular}

\captionsetup{justification=centering}
\caption{The histograms of Pods creation time with different number of Pods and different number of reconciling worker threads.}
\label{fig:pull-net-perf}}

\begin{flushleft}
{\it The figures show histograms of pod creation latencies for different configurations. From the first row to the last row are: (i)~25/50/100 tenants create 1250 pods, with each tenant creates random number of pods in the range of [40,60]/[20,30]/[10,15]; (ii)~25/50/100 tenants create 2500 pods, with each tenant creates random number of pods in the range of [75,125]/[40,60]/[20,30]; (iii)~25/50/100 tenants create 5000 pods, with each tenant creates random number of pods in then range of [160,240]/[75,125]/[40,60]; (iv)~25/50/100 tenants create 10000 pods, with each tenant creates random number of pods in a range of [300,500]/[150,250]/[75,125].}
\end{flushleft}
\end{figure*} 


==> pod-creation-statistics.tex <==
\begin{table*}[t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Configuration &
  \begin{tabular}[c]{@{}c@{}}25 Tenants\\ Baseline\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}25 Tenants\\ 20 Workers\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}25 Tenants\\ 100 Workers\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}50 Tenants\\ Baseline\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}50 Tenants\\ 20 Workers\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}50 Tenants\\ 100 Workers\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}100 Tenants\\ Baseline\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}100 Tenants\\ 20 Workers\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}100 Tenants\\ 100 Workers\end{tabular} \\ \hline
\multicolumn{10}{|c|}{1250 Pods}                                                                                   \\ \hline
Throughput (pods/secs)                             & 1250 & 625  & 416  & 1250 & 416   & 416  & 625  & 312  & 416  \\ \hline
Avg Creation Time (seconds)                        & 0.31 & 1.59 & 1.36 & 0.13 & 1.10  & 0.97 & 0.49 & 1.18 & 1.27 \\ \hline
\multicolumn{1}{|l|}{99\% Creation Time (seconds)} & 1.0  & 2.0  & 2.0  & 1.0  & 2.0   & 2.0  & 1.0  & 3.0  & 2.0  \\ \hline
\multicolumn{10}{|c|}{2500 Pods}                                                                                   \\ \hline
Throughput (pods/secs)                             & 833  & 416  & 500  & 833  & 833   & 625  & 625  & 416  & 357  \\ \hline
Avg Creation Time (seconds)                        & 0.62 & 2.20 & 2.41 & 0.5  & 2.11  & 1.95 & 0.74 & 2.02 & 2.21 \\ \hline
99\% Creation Time (seconds)                       & 2.0  & 5.0  & 4.0  & 2.0  & 7.0   & 2.0  & 2.0  & 4.0  & 4.0  \\ \hline
\multicolumn{10}{|c|}{5000 Pods}                                                                                   \\ \hline
Throughput (pods/secs)                             & 625  & 416  & 384  & 625  & 416   & 454  & 500  & 454  & 416  \\ \hline
Avg Creation Time (seconds)                        & 2.35 & 4.39 & 3.83 & 2.60 & 4.21  & 4.00 & 3.67 & 3.84 & 3.45 \\ \hline
99\% Creation Time (seconds)                       & 7.0  & 9.0  & 8.0  & 6.0  & 8.0   & 8.0  & 8.0  & 6.0  & 7.0  \\ \hline
\multicolumn{10}{|c|}{10000 Pods}                                                                                  \\ \hline
Throughput (pods/secs)                             & 555  & 434  & 434  & 555  & 454   & 454  & 555  & 434  & 434  \\ \hline
Avg Creation Time (seconds)                        & 6.54 & 9.23 & 9.22 & 6.81 & 8.94  & 8.27 & 4.7  & 7.16 & 8.04 \\ \hline
99\% Creation Time (seconds)                       & 15   & 19   & 19   & 16   & 17.01 & 17.0 & 8.0  & 14.0 & 15   \\ \hline
\end{tabular}%
}
\captionsetup{justification=centering}
\caption{The statistics of creating 10000 pods with different number tenants and reconciling worker threads.}
\label{fig:10k-pods-statistics}
\end{table*}


==> resource-usage.tex <==
\begin{figure}
{\centering
\begin{tabular}{c@{}c}
\includegraphics[width=0.5\linewidth]{25tenants_cpu.png} & \includegraphics[width=0.5\linewidth]{25_tenants_peak_mem.png} \\
\includegraphics[width=0.5\linewidth]{50tenants_cpu.png} & \includegraphics[width=0.5\linewidth]{50_tenants_peak_mem.png} \\
\includegraphics[width=0.5\linewidth]{100tenants_cpu.png} & \includegraphics[width=0.5\linewidth]{100_tenants_peak_mem.png} \\
\end{tabular}

\captionsetup{justification=centering}
\caption{The Resource Utilization of the Syncer Container}
\label{fig:syncer-rsrc-use}}

\begin{flushleft}
{\it The figures show the CPU and memory usage of the syncer container when creating 1250, 2500, 5000 and 10000 Pods. From the first row to the last row are results of 25, 50 and 100 tenants.}
\end{flushleft}
\end{figure}

